Bilocal geodesic operators as a tool of investigating the optical properties of spacetimes

In my thesis, I present one particular example of the formalism capable of describing the propagation of a family of light rays in a curved spacetime. It is based on the resolvent operator of the geodesic deviation equation for null geodesics which is known as the bilocal geodesic operator (BGO) formalism. The BGO formalism generalizes the standard treatment of light ray bundles by allowing observations extended in time or performed by a family of neighbouring observers. Furthermore, it provides a more unified picture of relativistic geometrical optics and imposes a number of consistency requirements between the optical observables. The thesis begins with a brief introduction of the transfer matrix and its relativistic versions known as the Jacobi propagators and the bilocal geodesic operators. Then the basics of differential geometry are reviewed, with an emphasis on the geometry of the tangent bundle and the geodesic flow, which later provide the foundation for the BGO formalism. The mathematical introduction is then followed by two articles about the applications of the BGO formalism in the studies of optical distance measures and the conclusion.

==> prel <==
Preliminaries:

*introduce the math machinery:
-tangent bundle TM (set of initial data; coordinate and vector; phase space in 1st order)
-tangent space to TM (variations of initial data)
-horizontal/vert subspaces(translation of notion of covariant derivative in this; vertical - position fixed, direction perturbed; horizontal - position changed with minimal effect on direction)
(covariant perturbation gives us coordinate-invariant observables)
(geodesic flow on TM; we can think of fluid in higher dim described by positions and momenta and we can)
(this way we connect to canonical formalism of Ham mechanics and phase space approach - thanks to canonical isomorphism)
(GDE - direct connection to curvature, captures and links it to geometric optics, deformation of shapes)(formally - a solution, link observation and emission regions, related to deformation tensor)

*justify why we use it

Big picture: BGO formalism is more general than what people have been using
|
|
----> drifts, parallax, image distorsion - all in one formalism.
|
|
|
----> provides links between all 3

~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
Notation (can be a bit difficult)(work with coordinate charts)

---------> points : p, x^\mu - from M to R^4

---------> covariance (x^\mu, v^\mu) from TM to R^8

---------> x^\mu from (x^\mu, v^\mu) from TM to R^4

---------> subtle distinction x^\mu

---------> element of T_(p, X_p)TM = # ddx + # ddv - coordinate dependent. An coord-ind description provided by Riemannian structure

---------> in a coord-ind way we can decompose T_(p, X_p)TM into H and V which are isomorphic to T_p M; so we can think of vectors in T_(p, X_p)TM as pairs of vectors telling us how to displace a point and perturb a tangent vector.

